Resource-Aware Automata and Games for Optimal Synthesis

We consider quantitative notions of parity automaton and parity game aimed at modelling resource-aware behaviour, and study (memory-full) strategies for exhibiting accepting runs that require a minimum amount of initial resources, respectively for winning a game with minimum initial resources. We also show how such strategies can be simplified to consist of only two types of moves: the former aimed at increasing resources, the latter aimed at satisfying the acceptance condition.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{J. Leroux and J.-F. Raskin (Eds.): Tenth International Symposium\\ on Games, Automata, Logics, and Formal Verification (GandALF'19).\\
EPTCS 305, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.305.4}{10.4204/EPTCS.305.4}}

